Pre-training via Paraphrasing

We introduce MARGE, a pre-trained sequence-to-sequence model learned with an unsupervised multi-lingual multi-document paraphrasing objective. MARGE provides an alternative to the dominant masked language modeling paradigm, where we self-supervise the reconstruction of target text by retrieving a set of related texts (in many languages) and conditioning on them to maximize the likelihood of generating the original. We show it is possible to jointly learn to do retrieval and reconstruction, given only a random initialization. The objective noisily captures aspects of paraphrase, translation, multi-document summarization, and information retrieval, allowing for strong zero-shot performance on several tasks. For example, with no additional task-specific training we achieve BLEU scores of up to 35.8 for document translation. We further show that fine-tuning gives strong performance on a range of discriminative and generative tasks in many languages, making MARGE the most generally applicable pre-training method to date.

==> other_content.tex <==
\subsubsection{XNLI}

\begin{table*}[]
\begin{tabular}{rrrrrrrrrrrrrrrrr}
\toprule
 & en & ar & bg & de & el & es & fr & hi & ru & sw & th & tr & ur & vi & zh & avg \\
\midrule
mBERT & 80.8 & 64.3 & 68.0 & 70.0 & 65.3 & 73.5 & 73.4 & 58.9 & 67.8 & 49.7 & 54.1 & 60.9 & 57.2 & 69.3 & 67.8 & 65.4 \\ 
MMTE & 79.6 & 64.9 & 70.4 & 68.2 & 67.3 & 71.6 & 69.5 & 63.5 & 66.2 & 61.9 & 66.2 & 63.6 & 60.0 & 69.7 & 69.2 & 67.5 \\ 
XLM & 82.8 & 66.0 & 71.9 & 72.7 & 70.4 & 75.5 & 74.3 & 62.5 & 69.9 & 58.1 & 65.5 & 66.4 & 59.8 & 70.7 & 70.2 & 69.1 \\
XLM-R & 88.7 & 77.2 & 83.0 & 82.5 & 80.8 & 83.7 & 82.2 & 75.6 & 79.1 & 71.2 & 77.4 & 78.0 & 71.7 & 79.3 & 78.2 & 79.2 \\ 
\midrule
\marge \\
\bottomrule
\end{tabular}
\caption{\textbf{XNLI}}
\end{table*}

\begin{table*}[]
\begin{tabular}{rcccccccc}
\toprule
  & en & ar & de & es & hi & vi & zh & avg \\
mBERT & 80.2 / 67.0 & 52.3 / 34.6 & 59.0 / 43.8 & 67.4 / 49.2 & 50.2 / 35.3 & 61.2 / 40.7 & 59.6 / 38.6 & 61.4 / 44.2 \\
MMTE & 78.5 / – & 56.1 / – & 58.4 / – & 64.9 / – & 46.2 / – & 59.4 / – & 58.3 / – & 60.3 / 41.4 \\
XLM & 68.6 / 55.2 & 42.5 / 25.2 & 50.8 / 37.2 & 54.7 / 37.9 & 34.4 / 21.1 & 48.3 / 30.2 & 40.5 / 21.9 & 48.5 / 32.6 \\
XLM-R & \bf{83.5} / \bf{70.6} & \bf{66.6} / \bf{47.1} & \bf{70.1} / \bf{54.9} & \bf{74.1} / \bf{56.6} & \bf{70.6} / \bf{53.1} & \bf{74.0} / \bf{52.9} & 62.1 / 37.0 & \bf{71.6} / \bf{53.2} \\
\midrule
\marge & 83.4 / 70.3 & 63.5 / 42.5  & 68.3 / 52.7 & 72.7 / 54.1 &67.2 / 49.2 & 70.9 / 48.9 & \bf{67.1} / \bf{43.6} & 70.6 / \\
\bottomrule
\end{tabular}
\caption{\label{table:mlqa}F1/Exact Match results for question answering on MLQA. Non-English results use zero-shot transfer learning. \marge performs competitively with XLM-R, with a fraction of the pre-training compute.
Comparison results are taken from \citet{xtreme}---with a different fine-tuning procedure \citet{xlmr} reports similar numbers to ours using XLM-R (average 70.7F1).
}
\end{table*}

\begin{table*}[]
\begin{tabular}{@{}llll@{}}
\toprule
           & \multicolumn{1}{c}{SQuAD} & \multicolumn{1}{c}{MNLI} & PAWS \\ \midrule
BERT Large &                           &                          &      \\
XLM-R      &                           &                          &      \\
BART       &                           &                          &      \\
mBART      & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{}     &      \\
MARGE      & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{}     &      \\
MARGE Wiki &                           &                          &      \\ \bottomrule
\end{tabular}
\caption{\textbf{Classification performance} on English question answering, entailment and paraphrasing tasks.}
\end{table*}



\begin{table*}[]
\begin{tabular}{rcccccccc}
\toprule
  & en & ar & de & es & hi & vi & zh & avg \\
  \midrule
mBERT & 80.2 & 52.3 & 59.0 & 67.4 & 50.2 & 61.2 & 59.6 & 61.4  \\
MMTE & 78.5 & 56.1 & 58.4 & 64.9 & 46.2 & 59.4 & 58.3 & 60.3 \\
XLM & 68.6 & 42.5 & 50.8 & 54.7 & 34.4 & 48.3 & 40.5 & 48.5  \\
XLM-R & \bf{83.5} & \bf{66.6} & \bf{70.1} & \bf{74.1} & \bf{70.6} & \bf{74.0} & 62.1 & \bf{71.6}  \\
\midrule
\marge & 83.4 & 63.5 & 68.3 & 72.7 &67.2 & 70.9 & \bf{67.1}& 70.6 \\
\bottomrule
\end{tabular}
\caption{\label{table:mlqa}F1 scores for question answering on MLQA. Non-English results use zero-shot transfer learning. \marge performs competitively with XLM-R, with a fraction of the pre-training compute.
Comparison results are taken from \citet{xtreme}---with a different fine-tuning procedure \citet{xlmr} reports similar numbers to ours using XLM-R (average 70.7F1).
}
\end{table*}


\begin{table*}[]
\begin{tabular}{rcccccccc}
\toprule
  & en & de & es & fr & ja & ko & zh & avg \\
\midrule
mBERT & 94.0 & 85.7 & 87.4 & 87.0 & 73.0 & 69.6 & 77.0 & 81.9 \\
MMTE & 93.1 & 85.1 & 87.2 & 86.9 & 72.0 & 69.2 & 75.9 & 81.3 \\
XLM & 94.0 & 85.9 & 88.3 & 87.4 & 69.3 & 64.8 & 76.5 & 80.9 \\
XLM-R & \bf{94.7} & \bf{89.7} & 90.1 & 90.4 & 78.7 &  \bf{79.0} & 82.3 & 86.4 \\
\midrule
\marge & \bf{94.7} & 89.4 & \bf{91.6} & \bf{90.9} & \bf{78.9}& 77.7 & \bf{82.5}& \bf{86.5}\\
\bottomrule
\end{tabular}
\caption{\label{table:pawsx}\textbf{PAWS-X} \marge outperforms previous work on cross-lingual transfer on the PAWS-X paraphrasing dataset.}
\end{table*}


==> retrieval_figure.tex <==


